Aligning Stuttered-Speech Research with End-User Needs: Scoping Review, Survey, and Guidelines

Atypical speech is receiving greater attention in speech technology research, but much of this work unfolds with limited interdisciplinary dialogue. For stuttered speech in particular, it is widely recognised that current speech recognition systems fall short in practice, and current evaluation methods and research priorities are not systematically grounded in end-user experiences and needs. In this work, we analyse these gaps through 1) a scoping review of papers that deal with stuttered speech and 2) a survey of 70 stakeholders, including adults who stutter and speech-language pathologists. By analysing these two perspectives, we propose a taxonomy of stuttered-speech research, identify where current research directions diverge from the needs articulated by stakeholders, and conclude by outlining concrete guidelines and directions towards addressing the real needs of the stuttering community.

==> old_content.tex <==
\section{Introduction}
\ztedit{In the past few years there has been an increase in research attention to modelling atypical speech~\cite{valente25_interspeech,Mujtaba2024InclusiveAF}---e.g., in automatic speech recognition (ASR), speech synthesis, and event classification.} Colin et al.~\cite{Lea2023FromUP} surveyed perceptions of People Who Stutter (henceforth, \pws) about speech recognition systems and provided recommendations for building better user-centric tools, specifically for voice-assistant systems. Jingjin et al. \cite{Li2025GovernWN} conducted a survey involving the stuttering community about data governance preferences for speech AI and derived best practices for ethical data collection, sharing, and use, underscoring that the community is both engaged and opinionated about how speech technology should be built. These works explore \pws~perception and needs from \emph{specific} stuttered speech technology. In contrast, we analyse the alignment between the broader stuttered-speech AI research landscape and end-user needs. End-user in this work refer to \pws~ and Speech Language Pathologists (henceforth, \slp). We ask four questions:

\begin{enumerate}
        \item \textit{What research areas do current stuttered-speech \ztedit{research} papers prioritise?}
         \item \textit{What do \pws~and \slp~say they need from voice-based \ztedit{systems}?}
         \item \textit{Where do the stakeholder needs and priorities align or conflict with research areas?}
         \item \textit{What are the implications of current research practices?} 
\end{enumerate}

Qualitative studies of everyday failures~\cite{Lea2023FromUP,Li2025OurCV} and quantitative evaluations of off-the-shelf models~\cite{mujtaba-etal-2024-lost,Mitra2021AnalysisAT} have shown that mainstream ASR systems under-perform on stuttered speech. Beyond these technical gaps, we are also motivated by the limited depth of stakeholder collaboration reported in prior work. While researchers often engage with stakeholders in corpus creation, we find that relatively few studies report stakeholder participation in problem formulation, task definition, annotation design, evaluation, or interpretation of system errors. Yet, end users are uniquely positioned to align model outputs with decision contexts, anticipate deployment constraints and harms, and articulate what ``\emph{useful}'' actually means in practice. Without systematically incorporating these points of view, it is difficult to ensure clinical relevance, problem–solution fit, ecological validity, and real-world transferability, or to prioritise requirements for truly human-centred design~\cite{Li2025OurCV,Sridhar2025JjjjustSB}.

\begin{figure}[t]
    \centering
    \includesvg[width=1\linewidth]{images/new_identification}
    \caption{Variation in inputs, task formulation and outputs for the Stutter Identification research area. We propose a task taxonomy (see Section \ref{sec:ResearchAreas}) to handle variation in output forms and standardize research nomenclature.}
    \label{fig:identification}
    \vspace{-1.5em}
\end{figure}

 We argue that these technical ASR gaps arise from limited stakeholder involvement in experiment design and evaluation for a ``correct'' ASR output, resulting in models optimised for generic benchmarks rather than clearly defined, user-centric use-cases. We find through a \textbf{user survey} and a \textbf{scoping review }that there is a discrepancy between what is desired by end users and what is addressed in stuttered-speech research. For example, \slp prefer transcripts that are true to produced speech for assessment and documentation, while \pws favour transcripts that represent intended speech for communication support. 

We also find that ambiguities arise around task \emph{naming} e.g., stutter \emph{detection} versus \emph{classification}. Without clear, shared task names and definitions, it is hard for the research community and stakeholders to know which output format a given system is optimising for, or to design benchmarks that separately and fairly evaluate either forms. 
We therefore, propose a \textbf{novel task taxonomy} that makes these distinctions explicit, so that user-centric objectives are targeted and measured effectively in research.




These issues are particularly important given the nature of stuttering itself. \hanan{something about ordering of the points in the introductions seems off}
Stuttering is a variable, multidimensional speech disorder that disrupts speech fluency leading to the occurrence of different \emph{stuttering events}. 
\ztdelete{in clinical practice, \slp need to quantify and characterize such events for screening, diagnoses, assessment, and \ztdelete{potential treatments development}\ztedit{developing treatment plans}.} Stuttering events are speech disruptions that can typically be described as repetitions, prolongations or blocks~\cite{valente25_interspeech}. 
These events vary among \pws in intensity and frequency and are typically used as a measure of severity. 
They are inherently multi-modal, extending beyond the occurrence of disruptions in the flow of speech to include facial and extremity movements. 
\ztedit{In clinical practice, \slp need to quantify and characterize such events for screening, diagnoses, assessment, and \ztdelete{potential treatments development}\ztedit{developing treatment plans}.} 
In stuttered-speech literature, however, the term \emph{\dq{disfluency events}} is often used to describe the stuttering events observable in the \emph{produced speech only}. 
Recent work by Valente et al.~\cite{valente25_interspeech}, for example, introduced new clinical-informed annotations for stuttering events in existing corpora, illustrating the need for agreeing on operational definitions. 


To answer these questions, we combine evidence from literature and stakeholders. Our contributions are: (i) we map $228$ stuttered-speech \ztedit{research} papers using our proposed task taxonomy and annotations for language coverage, stakeholder collaboration, and open science practices, (ii) we establish stakeholder needs, priorities and pain points through the user survey results from $40$ \pws and $30$ \slp, (iii) we analyse the alignment between state of stuttered-speech research and established stakeholder needs to identify systematic gaps, opportunities and implications, and (iv) we finally translate the findings into \ztdelete{actionable}\ztedit{concrete} recommendations for future research directions, evaluation practice and interdisciplinary protocols aimed at making stuttered-speech AI truly user-centred.




%\ztdelete{Research on atypical speech modelling has increased in recent years with research done on mainstream tasks like automatic speech recognition (ASR), speech synthesis and event detection/classification.}%\ZC{there should be more of an intro here before we go into the issues. Like what is the task etc.}
 % In contrast, we analyse the alignment between the broader stuttered-speech AI research landscape and end-user needs by asking four questions:
% Against this background, in this paper, w


% To better understand how stuttered-speech research \emph{aligns} with user-specific needs, we conduct scoping review of $228$ papers on stuttered-speech and conduct a survey of $2$ stakeholders; (i) Persons Who Stutter (\pws) and (ii) Speech Language Pathologists (\slp).

% A common theme is that research outputs sometimes have unclear clinical impact or use-cases, and that a single underlying model may be expected to serve very different needs: for example, \emph{\slp prefer transcripts that are true to produced speech for assessment and documentation, while \pws favour transcripts that represent intended speech for communication support}. These divergent stakeholder expectations show up in research at the level of modelling design choice and evaluation decision for a ``correct'' ASR output. 
% Yet, 

% \ZC{rewrote this before I got ot the end of the section, but we shouldn't include anything that we do or argue in before we have finished the motivation. Our position and arguments should come after we set up the problem space.}


%\ztdelete{However, we argue that stuttered, and more broadly, disfluent speech remains underserved by current atypical speech AI; the task formulations and benchmarks that dominate the literature do not consistently align with stakeholder priorities or real downstream use-cases.
%In this work, we focus specifically on \emph{stuttering} atypical speech and on two primary stakeholder groups: (i) Persons Who Stutter (\pws) and (ii) Speech Language Pathologists (\slp).}
%\ztdelete{Existing research has already highlighted some issues in the current state of literature. Prior studies have shown that current mainstream speech recognition systems under-serve the stuttering community, through \textit{qualitative} accounts of everyday failures~\cite{Lea2023FromUP,Li2025OurCV} and \textit{quantitative} evaluations of off-the-shelf models~\cite{mujtaba-etal-2024-lost,Mitra2021AnalysisAT} on stuttered speech.}
% A common theme is that research outputs sometimes have unclear clinical impact or use-cases, and that a single underlying model may be expected to serve very different needs: for example, \emph{\slp prefer transcripts that are true to produced speech for assessment and documentation, while \pws favour transcripts that represent intended speech for communication support}. These divergent stakeholder expectations show up in research at the level of modelling design choice and evaluation decision for a ``correct'' ASR output. 
%
%\ztdelete{These issues are partly a consequence of limited stakeholder involvement in} 


% when \pws and \slp are not consulted about objectives and success criteria, models tend to be

% \zc{What are the ambiguities you're referring to here? I'm not sure I recognise any ambiguities mentioned before}


% To answer these questions, we combine evidence from both sides. We first establish stakeholder needs, priorities and pain points through survey results from $40$ \pws and $30$ \slp and map $228$ stuttered-speech AI papers using a task taxonomy and annotations for language coverage, stakeholder collaboration, and open-science practices. We then perform an \emph{alignment analysis} that explicitly compares these two views to identify systematic gaps and opportunities. 
%
% \ZC{Our arguments etc should come in the paragraph below.}

% \zc{Is this a finding of our work or is this a finding of prior work? \response{H} It's a finding from our work \response{Z} Okay, in that case this shouldn't come here, our findings can't be motivating for our work. :)} 

% Another motivation for this work stems from limited depth of collaboration with stakeholders beyond data collection. 
% While researchers often engage with stakeholders in corpus creation, relatively few studies report stakeholder participation in problem formulation, task definition, annotation design, evaluation, or interpretation of system errors.
% Yet stakeholders are uniquely positioned to align model outputs with decision contexts, anticipate deployment constraints and harms, and articulate what ``\emph{useful}'' actually means in practice. 
% Without systematically incorporating stakeholder opinions, it is difficult to ensure clinical relevance and problem–solution fit, ecological validity, real-world transferability, or to prioritise requirements for truly human-centred design~\cite{Li2025OurCV,Sridhar2025JjjjustSB}.

% \footnote{movement to make scientific research transparent and accessible.}

% \zc{This sounds like we should split this up. So our contributions are 1) a taxonomy that we map to, 2) annotations of lang coverage etc., 3) a survey to establish stakeholder needs and wants, 4)} Second, we perform an \emph{alignment analysis}\zc{this is a new term to me, is this some standard I haven't caught before? \response{H} alignment is common for LLM-human values, using it here to explain how research priorities maps to stakeholder needs \response{Z} Yeah I know it from that literature but it's new to me here. I'd consider rephrasing this. \response{H} Can you make some suggestions?} to identify systematic gaps, opportunities and implications. 
% Finally, we translate the findings into \ztdelete{actionable}\ztedit{concrete} recommendations for future research directions, evaluation practice and interdisciplinary protocols aimed at making stuttered-speech AI truly user-centred.



%\subsection{Paper Structure}%Alignment Analysis and : how we compare literature and stakeholders}
% To move beyond a stand-alone literature survey and a stand-alone stakeholder survey, we explicitly analyse alignment between them. For each major research area and sub-task type in our taxonomy (defined in Section~\ref{sec:ResearchAreas}), we (i) quantify research area attention using paper count from our 228-paper corpus (Section \ref{sec:literatureCount}),
% %use the quantitative counts from the 228-paper corpus(Section \ref{sec:literatureCount}) to characterise how much attention each area receives, 
% and (ii) quantify stakeholder priorities/needs using ratings from \pws and \slp on the usefulness of corresponding tool types and the frequency of related themes in their free-text responses (Section~\ref{sec:stakeholder needs}). We then interpret, for each area, where literature priorities and stakeholder needs converge and where they diverge.\ZC{Either this should come before, the last sentence of the previous paragraph is basically wrapping up the introduction, or we can save this for when we get into the mapping.}


\textbf{Paper Structure:}
The remainder of the paper is structured as follows. 
Section~\ref{sec:literatureFindings} maps the current research landscape for stuttered-speech AI, introducing our task taxonomy and summarising key patterns in research areas, language coverage, open science, and stakeholder involvement. 
Section~\ref{sec: surveyDesign} describes the design and methodology of our stakeholder surveys. 
Section~\ref{sec:stakeholder needs} presents stakeholder insights, detailing \pws and \slp experience with existing tools and what they say they need from voice-based AI. 
In Section~\ref{sec:alignment}, we bring these strands together in an alignment analysis, comparing literature versus stakeholder priorities and highlighting systematic gaps and design implications. 
Finally, Section~\ref{sec:conclusion} outlines our proposed roadmap of actionable recommendations for future research, evaluation, and interdisciplinary collaboration.

% \zc{Make sure to use ref instead of hardcoded numbers.}

% for future research, evaluation practices, and interdisciplinary collaboration.
 % discusses the implications of these gaps and














% \subsection{Literature Review Protocol}

% We excluded papers that are not open-source but didn't filter by popular speech conference venue as this leads to exclusion of over 70\% of the papers. The initial 680 pool of papers included papers written by SLPs for neuroscience journals which aree out of scope for this work (as we want to focus on what AI research does for atypical speech to enable speaking together) \hanan{Write this more precisely as inclusion/exclusion criteria. This feels chatty}. To identify papers relating to machine learning for stuttered speech, we first read through the abstracts of the papers. 



% The screening lead to a set of $228$ papers that were further annotated to identify the key \textbf{research areas}, \textbf{language coverage}, \textbf{stakeholder involvement} and \textbf{open-source availability}. The further annotation involved reading the whole paper by the authors. In the identification of key research areas, we realized research in stuttered speech often involved a combination of tasks. For example, a work focusing on stuttering event detection ,involves stuttered speech recognition and analysis of data augmentation strategies. Therefore, we labelled some papers with multiple research areas. \hanan{Again this should be described as annotation guidelines/criteria, rather than your thinking process.}
% \red{First 234, removed some papers that contain questionable content (doesn't match abstract / or sound more like a proposal than research) even though their abstract was fine.}


% \section{Terminology and Task Taxonomy}



% \hanan{I think this belongs to the introduction, not here. The paper is about stuttering, so this should be defined at the start.}


% \subsubsection{Search strategy}
% To get the initial pool of papers, we used a keyword-based paper selection method using the Semantic Scholar API\footnote{\url{https://www.semanticscholar.org/product/api}} to gather approximately $680$ papers. We used these search terms: \dq{disfluency/dysfluency} , \dq{stuttering/stutter}, \dq{recognition}, \dq{detection}, \dq{classification},\dq{artificial intelligence}, \dq{machine learning}. We also filtered by year to include papers from 2010 - 2025. The search was conducted on October 29, 2025. 
% % \hanan{be more precise: what were the search terms used? Gone with CSCC }

% \subsubsection{Inclusion/Exclusion Criteria}
% We included peer-reviewed articles and preprints that (i) proposed, analysed, or evaluated computational or machine-learning methods for stuttered speech, and (ii) were available as open-source publications (i.e., with accessible full text). We did not restrict inclusion by publication venue (e.g., major speech conferences); doing so would have removed more than 70\% of otherwise eligible papers. We excluded works whose primary focus was clinical, neurological, or behavioural (e.g., SLP-authored neuroscience or neurolinguistics articles) without a substantive AI or speech-technology component, since our goal is to characterise how AI research addresses atypical speech to enable “speaking together.”
% \subsubsection{Analysis}

% After the initial screening, we obtained a set of 234 papers. During full-text annotation, we excluded a small number of papers whose main content did not match the abstract or that read primarily as proposals rather than completed empirical work, resulting in a final set of 228 papers. Each of these 228 papers was read in full and manually annotated along four dimensions: research areas, language coverage, stakeholder involvement, and open-source availability. For research areas, we assigned one or more labels from our taxonomy (e.g., Stutter Identification, Speech Recognition, Data, Research-focused) to each paper, allowing multiple labels whenever a work made a substantive contribution in more than one area. For instance, a study on stuttering event detection that also systematically analysed data augmentation strategies was annotated as both Stutter Identification and Data. For language coverage, we recorded all spoken languages (and dialects) explicitly targeted in the data and experiments, annotating every language for which training or evaluation was reported. Stakeholder involvement captured whether and how key stakeholders (PWS or SLPs) were involved beyond serving as data sources/annotators, including roles in study design, evaluation, or interpretation of results. Finally, open-source availability indicated whether the paper released any datasets or corpus resources, trained models or checkpoints, and/or source code or scripts sufficient to reproduce the main experiments.

\section{Task Taxonomy}
This section contains definitions of the main and their sub research areas identified from literature for stuttered speech research. The main research areas were obtained through an iterative-reduction process; we first give a phrase to describe what's done in a research work. Then we cluster by thematic coding and merge until we obtain the 7 areas described below:

\input{tables/research_areas}

\subsubsection{Speech Recognition}
\label{sec: SpeechRecognition}

Speech recognition is a well-established research area; however, the literature survey shows significant performance variations between fluent and disfluent speech. Speech recognition is defined as a speech-to-text problem, where the desired output is transcriptions of spoken speech. Some advanced works can even transcribe non-word sounds produced during communication, such as filler words (e.g., \dq{uhm}), laughter, and chuckles. 
% Regrettably, most off-the-shelf models fail at transcribing stuttered speech accurately, with error rates increasing as stutter severity increases \cite{Mujtaba2025FineTuningAF}. 
We describe 2 sub-tasks for speech recognition: 

(1) \textit{Intended speech recognition}: here, the transcription is true to the intent of the speaker, with produced stutter events completely removed from the transcripts. A use-case for this sub task is in voice-activity commands or dictation tools. In research an example is when evaluating the machine-generated transcription of a read speech that includes stuttering moments, the reference transcription (ground truth) should be the read passage. 

(2)\textit{Verbatim speech recognition}: in this form, the transcription is true to the produced speech, where the syllables, filler words or stutter events produced as a result of stuttering are included in the machine-generated transcription \textit{(e.g. I $\backslash$r won \textbf{or} I $\prec$rep$\succ$ won \textbf{or} I I I won)}. \footnote{In this example $\backslash$r and $\prec$rep$\succ$ stands for repetition stutter event.}

% Evaluation of this form of recognition should use carefully labeled ground-truth text that includes these repeated/prolonged syllables, filler words or special tokens. 

\subsubsection{Stutter Identification}
\begin{figure}
    \centering
    \includesvg[width=1\linewidth]{images/identification}
    \caption{Variation in inputs, and outputs for the Stutter Identification Task.}
    \label{fig:identification}
\end{figure}

Stuttering identification involves determining the occurrence of stuttering events in produced speech. This is a research area with high degree of variability in terms of sub-tasks according to literature. The variability occurs from level of granularity of model outputs, model inputs, etc as shown in Figure \ref{fig:identification}. Based on the findings of the literature survey, we describe 3 sub-tasks for stuttering identification: 


(1) \emph{Disfluency Classification}: this refers to an audio clip to class mapping problem. In this sub-task there's some variability on the \textit{class} mapping, some works perform binary classification (\emph{01 in Figure \ref{fig:identification}}), others do multi class classification (\emph{03 in Figure \ref{fig:identification}}) and the rest do multi label classification (one audio clip is mapped to 1 or more stuttering events (\emph{04 in Figure \ref{fig:identification}})). Another variability comes in the number of classes (stuttering events) which varies depending on annotation for the dataset. 

(2) \textit{Disfluency Detection:} this refers to time-frame to class mapping. Similar to (1), but the identification is more fine-grained to the temporal (seconds/frame) occurrence level of the event. Given an audio clip, the task formulation involves identifying time-bound occurrences of stuttering events(\emph{05 and 06 in Figure \ref{fig:identification}}), sometimes at a binary level and other times at a multi-class level. 
 
(3) \textit{Stuttering Severity Assessment}: this refers to the task of assigning a severity label to an audio clip. The task could be framed as a regression (on a numerical scale \emph{05 and 06 in Figure \ref{fig:identification}}) or multi-class problem (mid, low, high).

All the subtasks described for identification can be framed in a multi-modal format, using textual and/or visual information to perform the task.

\subsubsection{Speech Enhancement}
This task involves improving stuttered attempts through attempts to remove disfluencies either from speech or transcription. We describe 2 sub-tasks for speech enhancement:

(1) \textit{Speech Correction:} this involves removing disfluent events from produced speech. 

(2) \textit{Transcript Correction} this involves removing disfluent events from disfluent transcriptions.

% In the literature, there's some variability on the events handled by proposed models. Some works focus on some types of stuttering events: often prolongations, fillers and blocks.

\subsubsection{Data}
This task refers to efforts towards improvements to data for research involving resource development and data augmentation. We describe 2 sub-tasks:

(1) \textit{Resource Curation:} refers to works that have described efforts to either produce real recordings of PWS or works that describe efforts to provide updated annotations to existing corpora to benchmark new tasks.

(2) \textit{Data Augmentation:} refers to work that proposed data augmentation strategies and methods for synthetic disfluent speech generation.  

\subsubsection{Translation} This describes research efforts towards methods for producing fluent translations from either disfluent speech or disfluent transcription.

\subsubsection{Research-focused/Stutter speech processing}
There are a number of works that are not application focused, they are more towards improving research outputs for stuttered speech. e.g works on forced alignment / uncertainty quantification.
\textit{Surveys/ Reviews }: This sub-research area encompasses works that attempt to summarize and review the state of the literature. 
\textit{Ethics:} This refers to work on the intersection of research and humans, involving works that identify biases in research for stuttered speech or works that involves describing user perspectives to AI tools.

\subsubsection{Therapy / Fluency Tools}
This refers to work/demos that proposes frameworks or applications for PWS. We classify into 2 sub-tasks: (1) Measurement: tools built for assessment or identification (2)Practice: tools built for fluency practice.


% \section{Multi-view Survey Design}

% \subsection{Stakeholder Survey Design}

% \subsubsection{PWS Survey.} 
% Their survey included 4 main sections with 35 questions. 

% \noindent\textbf{Demographic and Background Information:} Demographics (age,gender,country of residence, country of origin);languages spoken(native,others) and their fluency level;education level;employment status.

% \noindent\textbf{Stuttering Profile:}impact on professional activity; self-reported severity level, frequency; severity across spoken languages; correlation of severity with situation, person.

% \noindent\textbf{AI Tool Utility Measure:}Usefulness of tools (identified by problem formulation in literature survey) in their day-to-day life; rating likelihood of participation in research-focused activity

% \noindent\textbf{Use, Perception and Needs of Voice-based AI Tools:} Usage,familiarity,challenges and concerns about AI tools; Recommendations for future research and tool development

% \subsubsection{SLP Survey.}
% Their survey included 4 main sections with 38 questions. 

% \noindent\textbf{Demographics and Professional Profile:} Demographics (age,gender,country of practice); clinical practice languages and their fluency level; similarity of stuttering characteristics across languages,age groups;education level;years of experience;frequency of work with PWS.

% \noindent\textbf{Current Work Life and Challenges:} Challenges from working with PWS; challenges from day-to-day clinical life; willingness to discuss challenges with researchers.

% \noindent\textbf{AI Tool Utility Measure:} Usefulness of tools (identified by problem formulation in literature survey) in working with PWS; importance of inter-disciplinary collaboration and stage of collaboration; importance of a tools language generalizability.

% \noindent\textbf{Use of AI tools:} Usage, familiarity, perceived benefits of AI Tools; challenges and concerns of using AI tools; field readiness and confidence about using AI tools; needs and recommendations for development and integration of AI tools.


\subsection{Distribution Across Research Areas \& Intersections}

Figure \ref{fig:taskCombination} indicates that stuttered-speech AI research is overwhelmingly dominated by \textbf{stutter identification}, which appears in \textbf{169 papers} (\textit{far more than any other category}). The largest intersection (96 papers) consists of papers focused only on stutter identification. The next most common overlaps pair stutter identification with \textbf{data-centric} (n=24) and with \textbf{research-focused} work (n=23), after which intersection sizes drop rapidly (most combinations occur in fewer than $\approx13$ papers, with many appearing only once).  

This pattern suggests that, although there is a non-trivial number of cross-area projects (16 distinct combinations), the field is still largely organized around single-task studies. Moreover, fewer than 20\% of papers explicitly report inter-disciplinary collaboration with stakeholders, indicating that much of this \emph{“inter-research-area”} work remains technically focused rather than truly human-centred. \hanan{So far, the questionnaire and literature survey parts read as two independent papers. The order of explaining things is rather odd, it feels like jumping between two separate topics.}

% While the intersection distribution shows a strong tendency toward single-task studies, the frequency of intersections (16) indicates there's a lot of inter-research area work (research involving multiple areas) but out of the examined literature a fewer ($\prec 20\%$) reported inter-disciplinary collaboration (involving stakeholders).

% === ChatGPT rephrase, original below ====
Open science practices are also limited. Only \textbf{23} papers (about 10\%) report releasing code, models, or data. Among these, the distribution is: \textbf{Data-centric} ($n=12$), \textbf{Stutter Identification} ($n=4$), \textbf{Research-focused} ($n=2$), and \textbf{Speech Recognition} ($n=5$). The particularly low number of open-source stutter-identification papers is striking given that it is the most heavily studied area, and it constrains reproducibility and downstream user adoption.

% Only $23$ ( about $10\%$) of the reviewed papers report release of code/models/data. Of the open-source papers, by research area we have the following distribution: Data (n=12), Stutter Identification (n=4), Research-focused (n=2), Speech Recognition (n=5). The low number of open-source papers for Stutter Identification is unexpected since it's the most common research area.


% === ChatGPT rephrase, original below ====
Within the \textit{research-focused} category, we observe an uneven mix of sub tasks: Surveys/Reviews ($n=17$), Evaluation/Analysis ($n=19$), Ethics ($n=6$), Anonymization and Privacy ($n=2$), Generalization of models ($n=2$), and Explainable methods ($n=2$). Together, these numbers suggest a growing but still relatively small body of work that critically examines methods, ethics, and deployment, compared to the much larger emphasis on building new stutter-identification models.

% In the research-focused category, Surveys/Reviews (n=17); Evaluation/Analysis (n=19), Ethics (n=6), Anonymization and Privacy (n=2), Generalization of models (2), Explainable methods (n=2).

\subsection{Language Coverage and Resources}
\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{images/langDist.png}
    \caption{Languages Covered in Literature}
    \label{fig:langDist}
\end{figure}
The language distribution in the surveyed stuttered-speech AI literature is \textbf{highly skewed toward English}. English accounts for 152 papers, far exceeding the next most common languages: German (23) and Mandarin (17) and indicating that most modelling, benchmarking, and evaluation choices are implicitly optimized for high-resource languages.

A notable secondary pattern is \textbf{limited but visible} coverage of \textbf{South Asian languages}: Marathi (5) and Hindi (5) appear most often, with smaller counts for Tamil (3), Bengali (3), Telugu (2), Kannada (2), and single-paper representation for Assamese, and Malayalam. This suggests growing interest in stuttering technologies beyond English, but the evidence base remains small and fragmented across many languages.

There is also modest representation of other widely spoken languages: French (3) and Spanish (3) and very sparse coverage of Japanese (2) and several languages with only one paper each (e.g., Korean, Persian, Indonesian, Polish, Ukrainian). Finally, the presence of “Unclear” (16) highlights reporting gaps in the literature: a non-trivial fraction of papers do not explicitly state the language of the data.

% Overall, the distribution indicates that research is English-centric, with improving efforts into other languages and a need for more consistent reporting and broader language coverage. 
This focus on high-resource language also indicate implicit bias in design choices as often proposed models rely on vasts amount of synthetic resources, lexicon or large scale pre-trained models that are mostly only available for high resource languages.

In terms of resource availability, since stuttering is a clinical condition there's often concerns and limitations on public availability of developed resources. Most works develop in-house resources for training and testing their models. Of all papers under the data-centric research area less than half(n=12) report public availability of curated resource. Out of these English appears in 12 works ($\succ 50$hrs)\footnote{Including synthetic corpora\label{note1}}, Mandarin in 2 ($\succ 50$hrs)\footref{note1}, German in 1 (4.6hrs) and Indian languages (Hindi, Telugu, Bengali, Marathi and Assamese) is in 1 work with very limited size (2.5hrs)

% The distribution of reported hours of avaialable resources per language are : English 

% For example, \cite{Zhou2024StutterSolverEM}  proposed approaches requiring  speech-text alignments obtained using a forced alignment that requires phoneme transcriptions for training and is only currently available for some high resource languages

\textbf{Monolingual vs Multilingual Works:} Most stuttered-speech AI studies in current literature are \textbf{monolingual: 183 papers }use data in a single language, compared with only \textbf{25 multilingual} studies. There's relatively limited work on cross-lingual transfer, language-agnostic representations, or systems designed to operate robustly across languages.

\subsection{High Variability, Less Standards}

 While some works tend to distinguish between the 2 sub-tasks of speech recognition defined in Section~\ref{sec: SpeechRecognition} and explicitly identify their work's task formulation or rename the evaluation metric to identify which form they're evaluating, most works do not explicitly explain what form of recognition they are performing. 

The stuttering identification literature exhibits substantial methodological variability and little standardization in task formulation. Papers alternately frame the problem as \textbf{binary classification} (stutter vs. fluent) ($n=38$), \textbf{multi class classification} with \textit{widely varying label sets} ($n=88$; commonly 3–8 classes; sometimes tied to specific event taxonomies such as repetition types), or \textbf{multi label classification} ($n=7$). Granularity is also inconsistent: some studies classify fixed-length clips (e.g., $3$ or $5$ seconds) while others use utterance-level labels. 

% The term detection/classification is often used interchangeably for disfluency classification and it's often unclear from titles to understand what task is being done by the publication. Standardized task definitions makes it easier to identify and compare relevant literature. \textbf{72 papers} include \textit{\dq{Detection}} in their title but \textbf{only 6 of these papers} do actual detection task per our definition. With our standardized sub task definition, we identify additional variability in disfluency classes across datasets and proposed models.

Terminology further obscures comparability: \textit{\dq{detection}} and \textit{\dq{classification}} are often used interchangeably for disfluency identification work, and titles rarely make the actual task clear. Although \textbf{72 papers} include \textit{\dq{Detection}} in their title, only \textbf{6} of these perform a detection task under our definition. Standardized task definitions makes it easier to identify and compare relevant literature.

% In the Data research area, papers focusing on resource curation also often vary on granularity level of disfluent events labeled and form of transcription provided. Works report varying types of disfluent events, for example in some annotations, repetition disfluency is sometimes broken down to sub classes like word-level, phoneme-level or syllable-level repetition. There's also variation on number (3 to 8) of disfluent event types. Some works in other research areas sometimes collapse sub-classes in their modeling or exclude entire classes in their work without justification or clinical context.


In the \textit{Data-centric} research area, resource-curation papers likewise differ in the granularity of labeled disfluent events and the form of transcription provided. Repetition, for example, may be subdivided into word-, syllable-, or phoneme-level categories, and the total number of disfluency types found in literature ranges from 3 to 8. Downstream modeling papers sometimes collapse these subclasses or exclude entire categories without justification or clinical rationale. Together, these inconsistencies make it difficult to compare results and to relate computational work to clinically meaningful constructs.




\subsection{Over the Years}

\begin{figure}[h]
    \centering
    \includesvg[width=1\linewidth]{images/stakeholder_involvement}
    \caption{Number of papers published by year. PWS means papers involving PWS collaboration; SLPs means papers involving SLP collaboration; All means all papers published.}
    \label{fig:stakeholder_involvement}
\end{figure}
\noindent\textbf{Stakeholder Involvement}: From Figure \ref{fig:stakeholder_involvement}, we see variations but increase in level of stakeholder involvement in stuttered speech research. Form the survey 38 of the reviewed papers report stakeholder involvement. We find stakeholders are also collaborating in these ways: data curation (n=24), interview/user study respondents(n=2), expert opinions (n=3), evaluation(n=7) and clinical testing (3). The level of their involvement is often towards resource contribution with more recent works \cite{Birol2025IsTA,Zhang2025DeployingUS} reporting SLP involvement for clinical testing of AI tools.

\medskip

\noindent\textbf{Research Interest}: There's a significant rise in research for stuttered speech and the number of research areas and languages covered. Only $23$ ( about $10\%$) of the reviewed papers report release of code/models/data and these all fall in the year range of 2021 - 2025. Of the 32 papers in the data research area, $28 \%$ involves synthetic data generation all from the year range of 2021 - 2025. 




\section{Results: Stakeholder Surveys}

One of the main goals of this work is to understand how AI speech research can better serve the stakeholders, we design two survey questionnaires to face the two stakeholders separately to see the needs, concerns and challenges from different perspectives. We additionally conduct a survey of research papers published for AI for atypical speech, specifically \textbf{stuttering}.


\subsection{Stakeholder Surveys}

\subsubsection{Design}
We collaborated with two SLPs to develop and share an online survey across their network of SLPs and PWS. The questions were first designed by the SLPs based on their clinical and research expertise. Afterwards we incorporated more AI-view questions, the final draft of questions were reviewed by SLPs. Many of the questions had multiple choice options with a text input option to fill in their responses. We used open-ended text input for questions on needs, challenges and recommendations. The list of questions are published here.\footnote{\url{Anonymous link}} To better understand impact of tools available from research for the stuttering community, we assess the stakeholders' perceived usefulness towards the tools capabilities. Participants were asked to rate tools on a likert scale \textit{(1 = not useful at all, 5 = very useful)}, the tools were described by their output e.g.\textit{ A tool that transcribes true to spoken speech - I um s s stutter a lot}.

\textit{\textbf{Persons Who Stutter (PWS) questionnaire:}} This survey consisted of four main sections with 35 questions in total covering participants’ demographic and background information, stuttering profile, perceived utility of AI tools, and experiences with voice-based AI tools. 

% The demographic and background section asked about age, gender, country of residence and origin, languages spoken (native and others) with fluency levels, education level, and employment status. The stuttering profile section explored its impact on professional activity, self-reported severity and frequency, differences in severity across spoken languages, and how severity correlates with specific situations or people. The AI Tool Utility Measure assessed how useful literature-identified tools were in participants’ day-to-day lives and how likely they would be to take part in research-focused activities. Finally, the section on use, perception, and needs of voice-based AI tools examined participants’ usage and familiarity, challenges and concerns related to AI tools, and their recommendations for future research and tool development.

\textbf{Demographic and Background:} section about age, gender, country of residence and origin, languages spoken (native and others) with fluency levels, education level, and employment status.

\textbf{Stuttering Profile:} explored the impact of stuttering on professional activity, self-reported severity and frequency, differences in severity across spoken languages, and how severity correlates with specific situations or people.

\textbf{AI Tool Utility Measure:} assessed how useful literature-identified tools were in participants’ day-to-day lives and how likely they would be to take part in research-focused activities.

\textbf{Use, Perception and Needs of Voice-based AI Tools:} examined participants’ usage and familiarity, challenges and concerns related to AI tools, and their recommendations for future research and tool development.

\textit{\textbf{Speech-Language-Pathologist (SLP) questionnaire:}} The SLP questionnaire consisted of four main sections with 38 questions in total addressing respondents’ demographics and professional profile, current work life and challenges, the perceived utility of AI tools, and current AI tool use. 


\textbf{Demographics and Professional Profile:} collected information on age, gender, and country of practice, as well as clinical practice languages and fluency levels, perceived similarity of stuttering characteristics across languages and age groups, education level, years of experience, and how frequently they work with people who stutter.

\textbf{Current Work Life and Challenges:} explored difficulties encountered when working with people who stutter, challenges in day-to-day clinical practice, and willingness to discuss these challenges with researchers.

\textbf{AI Tool Utility Measure:} assessed how useful literature-identified tools would be for clinical work with PWS, the importance and stage of interdisciplinary collaboration, and the importance of tool language generalizability.

\textbf{Use of AI tools:} examined usage and familiarity, perceived benefits, challenges and concerns, field readiness and confidence in adopting AI tools, and respondents’ needs and recommendations for developing and integrating AI tools.

% The demographics and professional profile section collected information on age, gender, and country of practice, as well as clinical practice languages and fluency levels, perceived similarity of stuttering characteristics across languages and age groups, education level, years of experience, and how frequently they work with people who stutter (PWS). The current work life and challenges section explored difficulties encountered when working with people who stutter, challenges in day-to-day clinical practice, and willingness to discuss these challenges with researchers. The AI Tool Utility Measure assessed how useful literature-identified tools would be for clinical work with PWS, the importance and stage of interdisciplinary collaboration, and the importance of tool language generalizability. Finally, the use of AI tools section examined usage and familiarity, perceived benefits, challenges and concerns, field readiness and confidence in adopting AI tools, and respondents’ needs and recommendations for developing and integrating AI tools. \hanan{For these two sections, I am not sure running text is the best format. Kinda hard to follow.}
\subsubsection{Recruitment}
% , inclusion criteria
The survey ran over a 3 month period with 70 respondents (40 PWS; 30 SLPs). The survey was published in both English and Spanish; a suggestion from one of the SLPs to facilitate reaching a broader audience. The participants were recruited through the network of the SLPs involved in this work.

\hanan{How were the participants identified/recruited?}


% \subsubsection{Measures}


 % \hanan{This should be incorporated into section 2.1.1}

\subsubsection{Analysis}
We use quantitative summaries (percentage of responses) to present the survey responses from both stakeholders. We use thematic coding to extract key points and actionable points from the open-ended questions.


\subsection{PWS Results}

\subsubsection{Demographics}
In terms of demographics, we had predominantly male(n = 27) respondents with 13 identifying as female.  Participants were spread across several countries, with most living in Portugal (11/40; 27.5\%), the United Arab Emirates (9/40; 22.5\%), or Peru (9/40; 22.5\%). Smaller numbers came from Spain (3/40; 7.5\%), Mexico (2/40; 5\%), and single respondents from Cabo Verde, the United Kingdom, Uzbekistan, the United States, Argentina, and Chile (each 1/40; 2.5\%). Figure \ref{fig:pws_demo} shows the distribution of age and gender.
\begin{figure}[h]
    \centering
    \includesvg[width=1\linewidth]{images/PWS_demo}
    \caption{Gender and Age distribution of PWS Respondents.}
    \label{fig:pws_demo}
\end{figure}



\subsubsection{Variability \& Impact}
\begin{figure}[h]
    \centering
    \includesvg[width=1\linewidth]{images/StutterVariability}
    \caption{PWS Responses to likert scale stutter variation questions.}
    \label{fig:pws_variability}
\end{figure}

Around $93\%$ of PWS respondents speak at least 2 languages, while $30\%$ of respondents speak more than 3 languages. $57\%$ of respondents who reported variability in stuttering by languages reported it differs by native or other language, while others report stuttering is about the same in all languages they speak. 

Respondents generally rated their current stuttering severity as mild to moderate, with most selecting levels 2 or 3 on the 5-point scale and only a small minority endorsing the highest severity level. Responses from PWS highlighted both the everyday impact of stuttering and its substantial variability across contexts (\emph{questions and number of respondents shown in Figure \ref{fig:pws_variability}}).  When asked about work life, ratings clustered around the midpoints of the scale, indicating that stuttering typically has a moderate impact on job or professional activities rather than no impact or a uniformly severe impact. In contrast, responses to the variability questions showed a much stronger effect of context: the majority of participants reported that specific situations such as interviews, reading aloud, or formal conversations markedly increase their stuttering, with most endorsing levels 4 or 5. Similarly, many respondents indicated that the person they are speaking to such as a boss, family member, or stranger, also influences their stuttering intensity, again with higher ratings more common than low ones.

% \todoinline{SLP describe POV.}

\subsubsection{Use and Perception of AI Tools}

\noindent\textbf{Impatient ASR: Experiences with "\textit{Voice Assistant}" Tools:} About half \approxpct{42} of PWS reported not using any voice-based AI tools (e.g., speech-based assistants, dictation tools, transcription). However, out of the respondents that \emph{do use} these tools, many describe the tools as \dq{\textbf{not at all accessible / not very accessible}}. A recurring theme in the accessibility barriers they described is \emph{impatient} where the voice assistant systems do not accommodate the natural pauses, blocks or repetitions inherent in stuttering. One of the respondents responded:

\begin{displayquote}
    \textit{\dq{I would change the fact that they stop listening when you start stuttering that would be very helpful.}} -- \texttt{PWS}
\end{displayquote}

to the open-ended question "What features or improvements would make voice-based AI tools more inclusive and supportive for people who stutter?". Another respondent replied: 
\begin{displayquote}
    \textit{\dq{One that gives you more time to speak when you stutter.}} -- \texttt{PWS}
\end{displayquote}
to the open-ended question on what tools they need to improve stuttering. These technical failures lead to \textbf{frustration and anxiety}, causing many PWS to \emph{avoid using AI tools because it’s uncomfortable}.


\medskip

\noindent\textbf{Participation in Data Initiatives:}
On a \textit{1 (`no, never') to 5 (`yes, absolutely')} scale, \textbf{PWS reported similarly high willingness to donate stuttered speech data through both anonymous and non‑anonymous crowd‑sourcing initiatives} \textcolor{red}{Didn't ask for video}. Ratings were nearly identical across the two options: anonymous participation averaged 3.6 (median 4) and non‑anonymous participation averaged 3.7 (median 4). Among those who expressed a preference (i.e., gave different scores), \textbf{\approxpct{62} leaned toward anonymous participation}, suggesting anonymity matters for a subset of participants, but \textbf{overall willingness was strong and broadly comparable in both settings}.


\subsection{SLP Results}
\subsubsection{Demographics}
The vast majority of the SLP respondents identified as female (27/30), with only three males. Clinically, they reported working with a wide range of languages, though practice was clearly dominated by Spanish/Castilian: most clinicians used Spanish or Castilian alone or in combination with other languages, including Basque, Catalan, Portuguese, Italian, and English. Of the 9 out of 30 respondents that work with multiple languages, all have over 6 years experience in the speech pathology field and 4 have less than 6 years working with PWS in particular. They have all completed specialized training in stuttering. Countries of practice were mostly distributed across Spain and Portugal, with additional representation from several Latin American countries (Argentina, Mexico, Peru, Chile, Colombia, Paraguay) and Italy and Catalunya. Overall, two-thirds (20/30) reported more than 10 years of work as speech-language therapists, and one-third had over 20 years in the profession. Experience specifically with people who stutter (PWS) was more evenly distributed across career stages: while over half (16/30) had 0–5 years of PWS-focused experience, nearly half (14/30) reported at least 6 years working with this population, including a core group (6/30) with more than 10 years of PWS experience.

\section{Old  Writing.}

\subsubsection{Use and Benefits of AI tools}

\noindent\textbf{Perceived Clinical Benefits:} Overall, SLPs most often framed AI as a way to save time and increase clinical efficiency, while also supporting more objective analysis, better documentation, and research-ready data, with additional perceived value in innovative therapy materials and expanded access to care for PWS.

\begin{table}[h]
 \caption{Benefits, count of SLPs who want them from AI tools and the frequency(in perecentage) of their selection by SLPs.}
    \centering
    \resizebox{0.8\columnwidth}{!}{%
    \begin{tabular}{@{}lcc} \toprule
         \textbf{Benefit} & \textbf{Count} & \textbf{Percent}\\ \midrule
         Time efficiency	 & 22 & \approxpct{73}\\
        Access to innovative materials & 15 & $50\%$\\
       Easier data collection for research  & 12 & $40\%$\\
         Objectivity in analysis & 11 & \approxpct{37}\\
         Improved documentation & 7 & \approxpct{23}\\
         	More access for PWS to treatment & 6 & $20\%$\\
         Enhanced patient engagement & 4 & \approxpct{13}\\ \bottomrule
    \end{tabular}
     }
    \label{tab:clinical benefit}
\end{table}

\medskip

\noindent\textbf{Clinical AI Integration: Open but not `Ready':} When asked `\textit{In your opinion, how ready is the field of speech-language therapy for the integration of AI / Automation technologies?}', most SLPs feel their field is not ready to adopt AI in speech language therapy with \approxpct{43} neutral (a 3 on a scale of 1-5) responses, \approxpct{37} low-readiness (1-2) responses and only $20\%$ of the respondents feel their field is ready to adopt AI. In contrast, when asked `\textit{Have you ever used voice AI-based tools in your clinical or research practice?}' and given the four options: (a) Yes, regularly (b) Occasionally (c) No, but I am interested and (d) No, and I am not interested. All SLPs who do not use AI ($63\%$ of respondents) chose (c), indicating their openness to adopting AI tools.







\subsubsection{Concerns and Challenges}

\noindent\textbf{Explainable Methods, Interpretable Results:} With clinical adaptation of research outputs in mind, we ask SLPs how important is it to understand how the models work and why they flag audio segments as stuttering events. SLPs indicated a strong desire for transparency from a stuttering-event identification tool, \textbf{rating both knowing how the tool works and why specific segments are flagged as highly useful}. Ratings were consistently high for both items (range 3–5 only; no 1s or 2s). 

\medskip

\noindent\textbf{Interdisciplinary Collaboration - \emph{When not If}:} SLPs expressed very strong support for interdisciplinary (clinical+researcher) collaboration in developing and evaluating AI tools for stuttered speech. On the 1–5 importance scale, ratings were very high overall (mean = 4.50/5; median = 5):\approxpct{67} selected 5, indicating that most SLPs view clinical collaboration as essential rather than optional. They also overwhelmingly felt collaboration should begin early: $90\%$ said interdisciplinary work should start from the very beginning (problem identification and project planning). Only a small minority suggested later entry points; \approxpct{7} recommended starting during model development/training (involving decisions about explainability/interpretability), and $3\%$ suggested beginning during implementation/clinical validation.

\medskip

\noindent\textbf{Concerns from the Clinical Perspective:}  In the open-ended responses to \textit{What are current concerns you have with AI tools? }, SLPs most often worried about \textbf{misinformation and insufficient accuracy} (e.g., whether tools can reliably recognize stuttering and provide correct information) and \textbf{privacy/data protection} (how patient data are collected, stored, and used). Several also raised profession- and practice-related concerns, including \textbf{over‑reliance on AI or replacement of clinicians}, potential \textbf{bias}, and \textbf{misuse/misinterpretation}—particularly if patients access incorrect information or if tools are used by professionals without sufficient stuttering expertise. A minority (5/30) reported no current concerns or said they hadn’t thought about it yet. It is also worth noting that 4 out of the 5 who reported having no concerns also reported not using any AI tool in their professional life. Below are some of the open-ended responses:

\begin{displayquote}
    \textit{effectiveness and accuracy on recognizing stuttering for the AI-tool} -- \texttt{SLP} \\
    \textit{I would say my main concerns relate to ethics and data protection.} -- \texttt{SLP}
\end{displayquote}

When asked about concrete \textbf{limitations/challenges} experienced (multiple selections allowed), respondents typically identified several barriers at once (almost all selected 3 challenges). The most frequently selected challenges are listed in Table \ref{tab:clinical limitations}.

\begin{table}[h]
    \caption{Frequency of challenge selection by SLPs.}
    \centering
    \resizebox{0.8\columnwidth}{!}{%
    \begin{tabular}{@{}lc@{}} \toprule
         \textbf{Limitation/Challenge}  & \textbf{Percent}\\ \midrule
         Lack of accuracy/reliability  & $63\%$\\
        Ethical or privacy concerns  & $63\%$\\
       Lack of training to use them & $63\%$\\
         Technical difficulties / lack of support  & $57\%$\\
         High cost or restricted access  & $37\%$\\
         	Limited language coverage  & $20\%$\\ \bottomrule
    \end{tabular}
     }
    \label{tab:clinical limitations}
\end{table}





\subsection{Cross-Stakeholder Comparison}

\noindent\textbf{Nuances to \dq{\textit{Speech Recognition}}:} Both stakeholders want transcribed speech, however with differences on how it should be done. \textbf{PWS rated the intended‑speech tool as more useful overall than the verbatim tool}. They lean more towards \textit{intended speech recognition} where stuttering events like syllable/word repetitions are omitted in the automatic transcript. High usefulness ratings (4–5) were more common for intended‑speech transcription (\approxpct{43}) than for verbatim transcription ($20\%$), while low ratings (1-2) were less common ($30\%$ vs \approxpct{53}). On the other hand, \textbf{SLPs rated the verbatim (true-to-spoken) transcription tool as more useful overall than the intended‑speech tool}. Most SLPs rated verbatim transcription as highly useful (4-5: \approxpct{83}) versus \approxpct{57} for the intended transcription, and SLPs were much more likely to give a neutral “3” to intended‑speech transcription ($30\%$) than to verbatim transcription (\approxpct{7}).

\medskip

\noindent\textbf{Beyond \dq{\textit{Binary Classification}}:} While PWS and SLPs wants to know \textit{if} stuttering occurs in some recorded speech, knowing \textit{when/where} stuttering occurs in the speech has slightly higher reported utility. On a \textit{1 (`not useful at all') to 5 (`very useful')} scale, SLPs rated both tools as highly useful, with a modest preference for the tool that can \textbf{tell where stuttering occurs}. High usefulness ratings (4–5) were more common for the `where' tool ($90\%$) compared with the `if stuttering occurs' tool (\approxpct{77}), while low ratings (1–2) were equally uncommon (\approxpct{7} for each). Neutral ratings (3) were much more frequent for the 'if' tool (\approxpct{17}) than for the 'where' tool ($3\%$). Same behaviour is reported among PWS where high usefulness ratings (4–5) were common for both tools (\approxpct{58} for when/where vs $55\%$ for whether-only), but low ratings (1–2) were less frequent for the when/where tool ($15\%$) than for the whether-only tool ($25\%$). Among those who expressed a preference (gave different scores), \approxpct{65} of PWS and $80\%$ of SLPs preferred the \textit{when/where} tool, suggesting that added detail about timing/location is valued by many users, even though most rated the two tools similarly.

\medskip

\noindent\textbf{Fluency or Clinical Assistants:} Many PWS respondents want tools for fluency practice and improved communication. Below are some extracted responses to questions on what AI tools they would like:

\begin{displayquote}
\textit{Where, when I send an audio recording, it automatically corrects and removes or edits the stuttering.} -- \texttt{PWS} \\
\textit{A dynamic app with exercises that help regulate stuttering, that shows the moments or words where I stumble the most and helps me regulate them.} -- \texttt{PWS}
\end{displayquote}

\medskip
\noindent\textbf{Severity Assessment:}
SLPs would also like to measure severity assessment to track longitudinal improvement and scenarios outside the therapy sessions.This is necessary as stuttering severity changes depending on who, what and when. \emph{Who}: who PWS is conversing with.\emph{What}: what's the situation like - anxious. \emph{when}: a formal or informal scene

\begin{displayquote}
    \textit{An App that can tell you how much you stutter and for how long.} -- \texttt{PWS} \\
    \textit{AI tools that help me identify when I stutter.} -- \texttt{PWS}
\end{displayquote}










\section{Discussion}

\subsection{Alignment / Misalignment Between Stakeholder Needs and Current Literature}
While both stakeholders want to know \emph{if} (classification) stuttering occurs in a speech sample, the response also indicates a stronger preference for \emph{when and where} (detection) tool. There's a slight gap in current state of research, although the Stutter Identification task is the most popular, there's significantly more work on classification than detection and even less open-source models for identification.

In the current literature, an often overlooked fact is the difference in verbatim vs. intended speech recognition (survey response indicates both forms are useful depending on the stakeholder) where researchers are not explicit about which of the two forms they are optimizing for and often making implicit design choices that favor one form. Also, data resources often produce one form of transcript (intended) for the data from reading scenarios.

A less researched area is multi-linguality and language generalizability of models, survey response indicates most respondents are multilingual and stuttering varies by language. 

% Siloed Research: 
Research on fluency assistant tools often involve combination of works from multiple research areas, the current state of open-source avaialbility, variability and lack of standards makes it uneasy to test different approaches.  While 169 papers focus on Stutter Identification, only 15 focus on Therapy/Fluency Tools, this quantitatively proves the research is not application-focused.

% \textcolor{red}{Fluency assistants include a combination of technologies: ASR,TTS,conversation,speech analysis but models reporting SOTA individually are not open-source}


% \subsection{Implications for Task Definitions and Evaluation}

% \subsection{Implications for Language Coverage and  Generalizability}

% \subsection{Implications for Adaptation}




    % \item \textbf{Speech Recognition}: defined as a speech-to-text problem, where the desired output is transcriptions of spoken speech. We describe $2$ sub-tasks for speech recognition: (i) \textit{Intended speech recognition}: here, the transcription is true to the intent of the speaker, with produced stutter events completely removed from the transcripts. A use-case for this sub task is in voice-activity commands or dictation tools. In research an example is when evaluating the machine-generated transcription of a read speech that includes stuttering moments, the reference transcription (ground truth) should be the read passage. , and (ii)\textit{Verbatim speech recognition}: in this form, the transcription is true to the produced speech, where the syllables, filler words or stutter events produced as a result of stuttering are included in the machine-generated transcription \textit{(e.g. I $\backslash$r won \textbf{or} I $\prec$rep$\succ$ won \textbf{or} I I I won)}. \footnote{In this example $\backslash$r and $\prec$rep$\succ$ stands for repetition stutter event.}
    
    % \item \textbf{Stutter Identification}: involves determining the occurrence/intensity of stuttering events in produced speech. This task has high degree of variability in terms of sub-tasks according to literature. The variability occurs from level of granularity of model outputs, model inputs, etc as shown in Figure \ref{fig:identification}. We describe 3 sub-tasks for stuttering identification: (i) \textit{Stutter Classification} refers to an audio clip to class mapping problem. In this sub-task there's additional variability on the numer of \textit{class} mapping: binary classification (\emph{01 in Figure \ref{fig:identification}}), multi class classification (\emph{03 in Figure \ref{fig:identification}}) and, multi label classification (one audio clip is mapped to 1 or more stuttering events (\emph{04 in Figure \ref{fig:identification}})), (ii) \textit{Stutter Detection} describes time-frame to class mapping. Differs from (i) in that identification is more fine-grained to the temporal (seconds/frame) occurrence level of the event. Given an audio clip, the task formulation involves identifying time-bound occurrences of stuttering events, sometimes at a binary level and other times at a multi-class level (\emph{05 and 06 in Figure \ref{fig:identification}}), and (iii) \textit{Stuttering Severity Assessment}: this refers to the task of assigning a severity label to an audio clip. The task could be framed as a regression (on a numerical scale \emph{05 and 06 in Figure \ref{fig:identification}}) or multi-class problem (mid, low, high). All the subtasks described for identification can be framed in a multi-modal format, using textual and/or visual information for modelling.

    \ztedit{\subsubsection{Discussion}}
Overall, \ztdelete{these}\ztedit{our} findings \ztdelete{show}\ztedit{indicate} that the stuttered-speech \ztdelete{AI}\ztedit{technologies} field is active, but narrowly scoped. 
The literature is overwhelmingly organized around monolingual stutter classification tasks, with inconsistent task naming and an implicit default toward intended speech recognition. Stakeholder collaboration and open-science practices are still the exception rather than the rule, and work that investigates ethics, explainability, or deployment remains \ztdelete{comparatively} sparse. However, recent \ztdelete{output shows}\ztedit{trends give} encouraging signs: more papers \ztedit{are being published in the area}\ztdelete{overall}, \ztedit{there is} a gradual rise in stakeholder involvement, and open datasets and synthetic-data efforts, suggesting growing awareness of some of these \emph{technical}\hanan{Why the focus on technical? I don't see these are mainly technical issues;\response{H} using technical for lack of better term, I will find a different word} issues. However, fixing technical problems in isolation does not guarantee that systems will serve \pws~and \slp~well: some technical gaps are starting to close, but the extent to which the current state of research actually \emph{aligns with their needs}\hanan{There is heavy use of italics that I don't like, but maybe that's just me. I don't find it necessary to stress on specific phrases so much. \response{H} I like when points are emphasized, helps me to skim easily } remains an open question.
